GANSpace: Discovering Interpretable GAN Controls

This paper describes a simple technique to analyze Generative Adversarial Networks (GANs) and create interpretable controls for image synthesis, such as change of viewpoint, aging, lighting, and time of day. We identify important latent directions based on Principal Components Analysis (PCA) applied either in latent space or feature space. Then, we show that a large number of interpretable controls can be defined by layer-wise perturbation along the principal directions. Moreover, we show that BigGAN can be controlled with layer-wise inputs in a StyleGAN-like manner. We show results on different GANs trained on various datasets, and demonstrate good qualitative matches to edit directions found through earlier supervised approaches.

==> figures_arxiv_reduced/imgrid/imgrid.tex <==
\newcommand{\fwid}{1in}
\begin{figure}
\centering
	\includegraphics[width=\fwid]{gantest_-3_-3.jpg}\hfill%
	\includegraphics[width=\fwid]{gantest_-2_-3.jpg}\hfill%
	\includegraphics[width=\fwid]{gantest_-1_-3.jpg}\hfill%
	\includegraphics[width=\fwid]{gantest_0_-3.jpg}\hfill%
	\includegraphics[width=\fwid]{gantest_1_-3.jpg}\hfill%
	\includegraphics[width=\fwid]{gantest_2_-3.jpg}\hfill%
	\includegraphics[width=\fwid]{gantest_3_-3.jpg}
\\
	\includegraphics[width=\fwid]{gantest_-3_-2.jpg}\hfill%
	\includegraphics[width=\fwid]{gantest_-2_-2.jpg}\hfill%
	\includegraphics[width=\fwid]{gantest_-1_-2.jpg}\hfill%
	\includegraphics[width=\fwid]{gantest_0_-2.jpg}\hfill%
	\includegraphics[width=\fwid]{gantest_1_-2.jpg}\hfill%
	\includegraphics[width=\fwid]{gantest_2_-2.jpg}\hfill%
	\includegraphics[width=\fwid]{gantest_3_-2.jpg}
\\
	\includegraphics[width=\fwid]{gantest_-3_-1.jpg}\hfill%
	\includegraphics[width=\fwid]{gantest_-2_-1.jpg}\hfill%
	\includegraphics[width=\fwid]{gantest_-1_-1.jpg}\hfill%
	\includegraphics[width=\fwid]{gantest_0_-1.jpg}\hfill%
	\includegraphics[width=\fwid]{gantest_1_-1.jpg}\hfill%
	\includegraphics[width=\fwid]{gantest_2_-1.jpg}\hfill%
	\includegraphics[width=\fwid]{gantest_3_-1.jpg}
\\
	\includegraphics[width=\fwid]{gantest_-3_0.jpg}\hfill%
	\includegraphics[width=\fwid]{gantest_-2_0.jpg}\hfill%
	\includegraphics[width=\fwid]{gantest_-1_0.jpg}\hfill%
	\includegraphics[width=\fwid]{gantest_0_0.jpg}\hfill%
	\includegraphics[width=\fwid]{gantest_1_0.jpg}\hfill%
	\includegraphics[width=\fwid]{gantest_2_0.jpg}\hfill%
	\includegraphics[width=\fwid]{gantest_3_0.jpg}
\\
	\includegraphics[width=\fwid]{gantest_-3_1.jpg}\hfill%
	\includegraphics[width=\fwid]{gantest_-2_1.jpg}\hfill%
	\includegraphics[width=\fwid]{gantest_-1_1.jpg}\hfill%
	\includegraphics[width=\fwid]{gantest_0_1.jpg}\hfill%
	\includegraphics[width=\fwid]{gantest_1_1.jpg}\hfill%
	\includegraphics[width=\fwid]{gantest_2_1.jpg}\hfill%
	\includegraphics[width=\fwid]{gantest_3_1.jpg}
\\
	\includegraphics[width=\fwid]{gantest_-3_2.jpg}\hfill%
	\includegraphics[width=\fwid]{gantest_-2_2.jpg}\hfill%
	\includegraphics[width=\fwid]{gantest_-1_2.jpg}\hfill%
	\includegraphics[width=\fwid]{gantest_0_2.jpg}\hfill%
	\includegraphics[width=\fwid]{gantest_1_2.jpg}\hfill%
	\includegraphics[width=\fwid]{gantest_2_2.jpg}\hfill%
	\includegraphics[width=\fwid]{gantest_3_2.jpg}
\\
	\includegraphics[width=\fwid]{gantest_-3_3.jpg}\hfill%
	\includegraphics[width=\fwid]{gantest_-2_3.jpg}\hfill%
	\includegraphics[width=\fwid]{gantest_-1_3.jpg}\hfill%
	\includegraphics[width=\fwid]{gantest_0_3.jpg}\hfill%
	\includegraphics[width=\fwid]{gantest_1_3.jpg}\hfill%
	\includegraphics[width=\fwid]{gantest_2_3.jpg}\hfill%
	\includegraphics[width=\fwid]{gantest_3_3.jpg}
\caption{Caption TBD}
\label{fig:labelTBD}
\end{figure}

==> latexmkrc <==
###############################
# Post processing of pdf file #
###############################

# custom time zone
$ENV{'TZ'}='Europe/Helsinki';

# assume the jobname is 'output' for Overleaf v2
my $ORIG_PDF_AGE = -M "output.pdf"; # get age of existing pdf if present

END {
    my $NEW_PDF_AGE = -M "output.pdf";
    return if !defined($NEW_PDF_AGE); # bail out if no pdf file
    return if defined($ORIG_PDF_AGE) && $NEW_PDF_AGE == $ORIG_PDF_AGE; # bail out if pdf was not updated
    my $QPDF = "/usr/bin/qpdf";
    return if ! -x $QPDF; # check that qpdf exists
    my $status = system($QPDF, "--linearize", "output.pdf", "output.pdf.opt");
    my $exitcode = ($status >> 8);
    print "qpdf exit code=$exitcode\n";
    # qpdf returns 0 for success, 3 for warnings (output pdf still created)
    return if !($exitcode == 0 || $exitcode == 3);
    print "Renaming optimised file to output.pdf\n";
    rename("output.pdf.opt", "output.pdf");
}

##############
# Glossaries #
##############
add_cus_dep( 'glo', 'gls', 0, 'glo2gls' );
add_cus_dep( 'acn', 'acr', 0, 'glo2gls');  # from Overleaf v1
sub glo2gls {
	system("makeglossaries $_[0]");
}

#############
# makeindex #
#############
@ist = glob("*.ist");
if (scalar(@ist) > 0) {
        $makeindex = "makeindex -s $ist[0] %O -o %D %S";
}

################
# nomenclature #
################
add_cus_dep("nlo", "nls", 0, "nlo2nls");
sub nlo2nls {
	system("makeindex $_[0].nlo -s nomencl.ist -o $_[0].nls -t $_[0].nlg");
}

#########
# Knitr #
#########
my $root_file = $ARGV[-1];

add_cus_dep( 'Rtex', 'tex', 0, 'rtex_to_tex');
sub rtex_to_tex {
    do_knitr("$_[0].Rtex");
}

sub do_knitr {
    my $dirname = dirname $_[0];
    my $basename = basename $_[0];
    system("Rscript -e \"library('knitr'); setwd('$dirname'); knit('$basename')\"");
}

my $rtex_file = $root_file =~ s/\.tex$/.Rtex/r;
unless (-e $root_file) {
	if (-e $rtex_file) {
		do_knitr($rtex_file);
	}
}

##########
# feynmf #
##########
push(@file_not_found, '^feynmf: Files .* and (.*) not found:$');
add_cus_dep("mf", "tfm", 0, "mf_to_tfm");
sub mf_to_tfm { system("mf '\\mode:=laserjet; input $_[0]'"); }

push(@file_not_found, '^feynmf: Label file (.*) not found:$');
add_cus_dep("mf", "t1", 0, "mf_to_label1");
sub mf_to_label1 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t1"); }
add_cus_dep("mf", "t2", 0, "mf_to_label2");
sub mf_to_label2 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t2"); }
add_cus_dep("mf", "t3", 0, "mf_to_label3");
sub mf_to_label3 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t3"); }
add_cus_dep("mf", "t4", 0, "mf_to_label4");
sub mf_to_label4 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t4"); }
add_cus_dep("mf", "t5", 0, "mf_to_label5");
sub mf_to_label5 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t5"); }
add_cus_dep("mf", "t6", 0, "mf_to_label6");
sub mf_to_label6 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t6"); }
add_cus_dep("mf", "t7", 0, "mf_to_label7");
sub mf_to_label7 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t7"); }
add_cus_dep("mf", "t8", 0, "mf_to_label8");
sub mf_to_label8 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t8"); }
add_cus_dep("mf", "t9", 0, "mf_to_label9");
sub mf_to_label9 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t9"); }

##########
# feynmp #
##########
push(@file_not_found, '^dvipdf: Could not find figure file (.*); continuing.$');
add_cus_dep("mp", "1", 0, "mp_to_eps");
sub mp_to_eps {
    system("mpost $_[0]");
    return 0;
}

#############
# asymptote #
#############
sub asy {return system("asy --offscreen '$_[0]'");}
add_cus_dep("asy","eps",0,"asy");
add_cus_dep("asy","pdf",0,"asy");
add_cus_dep("asy","tex",0,"asy");

#############
# metapost  #  # from Overleaf v1
#############
add_cus_dep('mp', '1', 0, 'mpost');
sub mpost {
  my $file = $_[0];
  my ($name, $path) = fileparse($file);
  pushd($path);
  my $return = system "mpost $name";
  popd();
  return $return;
}

##########
# chktex #
##########
unlink 'output.chktex' if -f 'output.chktex';
if (defined $ENV{'CHKTEX_OPTIONS'}) {
    use File::Basename;
    use Cwd;

    # identify the main file
    my $target = $ARGV[-1];
    my $file = basename($target);

    if ($file =~ /\.tex$/) {
	# change directory for a limited scope
	my $orig_dir = cwd();
	my $subdir = dirname($target);
	chdir($subdir);
	# run chktex on main file
	$status = system(
    "/usr/bin/run-chktex.sh",
    $orig_dir,
    $file
  );
	# go back to original directory
	chdir($orig_dir);

	# in VALIDATE mode we always exit after running chktex
	# otherwise we exit if EXIT_ON_ERROR is set

	if ($ENV{'CHKTEX_EXIT_ON_ERROR'} || $ENV{'CHKTEX_VALIDATE'}) {
	    # chktex doesn't let us access the error info via exit status
	    # so look through the output
	    open(my $fh, "<", "output.chktex");
	    my $errors = 0;
	    {
		local $/ = "\n";
		while(<$fh>) {
		    if (/^\S+:\d+:\d+: Error:/) {
			$errors++;
			print;
		    }
		}
	    }
	    close($fh);
	    exit(1) if $errors > 0;
	    exit(0) if $ENV{'CHKTEX_VALIDATE'};
	}
    }
}
